A First Look at 5G Core Deployments on Public Cloud: Performance Evaluation of Control and User Planes

The Fifth Generation (5G) mobile core network is designed as a set of Virtual Network Functions (VNFs) hosted on Commercial-Off-the-Shelf (COTS) hardware. This creates a growing demand for general-purpose compute resources as 5G deployments continue to expand. Given their elastic infrastructure, cloud services such as Amazon Web Services (AWS) are attractive platforms to address this need. Therefore, it is crucial to understand the control and user plane Quality of Service (QoS) performance associated with deploying the 5G core on top of a public cloud. To account for both software and communication costs, we build a 5G testbed using open-source components spanning multiple locations within AWS. We present an operational breakdown of the performance overhead for various 5G use cases using different core deployment strategies. Our results indicate that moving specific VNFs into edge regions reduces the latency overhead for key 5G operations. Furthermore, we instantiated multiple user plane connections between availability zones and edge regions with different traffic loads. We observed that the deterioration of connection quality varies depending on traffic loads and is use case specific. Ultimately, our findings provide new insights for Mobile Virtual Network Operators (MVNOs) for optimal placements of their 5G core functions.

==> abstract.tex <==
%The Fifth Generation (5G) of mobile networks leverage Network Functions Virtualization (NFV) as a key enabler. 
%for scalability and flexibility. 
The Fifth Generation (5G) mobile core network is implemented as a set of Virtual Network Functions (VNFs) hosted on Commercial Off-the-Shelf (COTS) hardware. This design creates a growing demand for general-purpose compute resources as 5G network deployments continue to expand. Given their extensive infrastructures, public cloud services such as Amazon Web Services (AWS) are attractive platforms 
to fill this vacuum. 
%for Mobile Virtual Network Operators (MVNOs). 
Therefore, it is crucial to understand the control and user plane Quality of Service (QoS) implications associated with deploying a 5G core network on top of a public cloud. This analysis will assist Mobile Virtual Network Operators (MVNO) with infrastructural decisions. In our investigation, we construct a 5G testbed spanning multiple global locations (i.e., United States, Europe, Asia-Pacific) within the public AWS infrastructure.
%comprised of edge zone variants such as Local and Wavelength Zones. 
%within the AWS infrastructure. 
Integrated into this testbed is an HTTP transaction tracing framework built with state-of-the-art components and a custom monitoring Side-car Proxy (SCP). Using different core deployments strategies by shuffling VNFs into AWS edge zones, an operational breakdown of the latency bottlenecks is carried out for critical 5G procedures. Results show that moving specific VNFs into edge regions will lead to sub-10~ms latency for select operations of Mission Critical Services (MCSs). To evaluate user plane bottlenecks between edge zones and availability zones, we instantiate multiple 5G user plane connections with pre-recorded traffic patterns.
%across AWS 
%while measuring throughput and packet loss. 
Our results show that the majority of the edge zones operate at bandwidths below 200Mbps with over 25\% packet loss using a 1Gbps UDP connection. 
%The QoS for most regions in specific cities deteriorates significantly as more 5G data session are instantiated.

==> abstract2.tex <==
The Fifth Generation (5G) mobile core network has been implemented as a set of Virtual Network Functions (VNFs) hosted on Commercial Off-the-Shelf (COTS) hardware, which creates growing demand for general-purpose compute resources as 5G network deployments continue to expand. Given their existing infrastructures, cloud providers such as Amazon Web Services (AWS) are attractive platforms to fill this need.  Therefore, it is crucial to understand the control and user plane Quality of Service (QoS) implications associated with deploying a 5G core network on top of AWS. %in the near future. 
%In our investigation, 
To this end, we construct a 5G testbed with open-source components spanning multiple locations within the AWS infrastructure. %Integrated into this testbed is an HTTP transaction tracing framework built with state-of-the-art components and a custom monitoring Side-car Proxy (SCP). 
Using different core deployments strategies by shuffling VNFs into AWS edge zones, an operational breakdown of the latency overhead is conducted for 5G procedures. 
Results show that moving specific VNFs into edge regions lower the latency overhead for key operations. 
%Results show that moving specific VNFs into edge regions lead to sub-10~ms latency overhead for key operations. 
To evaluate user plane bottlenecks between edge zones and availability zones, we instantiate multiple 5G user plane connections with various traffic loads. As more data sessions are instantiated, we observe that the deterioration of the connection quality varies depending on the traffic load.
%Our results show that most of the edge zones operate at bandwidths below 200Mbps with over 25\% packet loss using a 1Gbps UDP connection.
Our work in this paper will assist Mobile Virtual Network Operators (MVNO) in determining favourable placements for their 5G core entities in the cloud.

==> abstract3.tex <==
The Fifth Generation (5G) mobile core network is implemented as a set of Virtual Network Functions (VNFs) hosted on Commercial-Off-the-Shelf (COTS) hardware. This creates growing demand for general-purpose compute resources as 5G deployments continue to expand. Given their existing infrastructures, cloud providers such as Amazon Web Services (AWS) are attractive platforms to address this need. Therefore, it is crucial to understand the control and user plane Quality of Service (QoS) implications associated with deploying the 5G core on top of AWS. %%%%%%%%% new sentence for focusing on AWS measurements
To this end, we conduct a thorough measurement campaign to understand the performance bottlenecks that exist between the central and edge AWS infrastructure. %%%%%%%%%
Furthermore, a 5G testbed is constructed with open-source components spanning multiple locations within AWS. Using different core deployment strategies by shuffling VNFs into AWS edge zones, an operational breakdown of the latency overhead is presented for various 5G procedures. Our results show that moving specific VNFs into edge regions reduces the latency overhead for key 5G operations. We instantiate multiple user plane connections between availability zones and edge regions with different traffic loads. As more data sessions are instantiated, we observe that the deterioration of connection quality varies depending on traffic load. Ultimately, our findings provide new insights for Mobile Virtual Network Operators (MVNO) to determine favorable placements of their 5G core entities in the cloud.

%shortened 4 words

%The Fifth Generation (5G) mobile core network is implemented as a set of Virtual Network Functions (VNFs) hosted on Commercial-Off-the-Shelf (COTS) hardware. This creates growing demand for general-purpose compute resources as 5G network deployments continue to expand. Given their existing infrastructures, cloud providers such as Amazon Web Services (AWS) are attractive platforms to address this need. Therefore, it is crucial to understand the control and user plane Quality of Service (QoS) implications associated with deploying the 5G core on top of AWS. To this end, we construct a 5G testbed with open-source components spanning multiple locations within the AWS infrastructure. Using different core deployments strategies by shuffling VNFs into AWS edge zones, an operational breakdown of the latency overhead is conducted for 5G procedures. Our measurement results show that moving specific VNFs into edge regions reduces the latency overhead for key 5G operations. We instantiate multiple user plane connections between availability zones and edge regions with different traffic loads. As more data sessions are instantiated, we observe that the deterioration of the connection quality varies depending on the traffic load. Ultimately, our findings provide new insights to Mobile Virtual Network Operators (MVNO) for determining favorable placements of their 5G core entities in the cloud.

==> ethics.tex <==
During our user plane evaluations, we generate high traffic volume through a 5G connection between AZs and our chosen set of edge zones. This occupies large chunks of bandwidth that can potentially deteriorate the performance of other applications using the same connection. However, we are essentially leveraging a paid service offered by AWS and therefore are charged the appropriate fees for our data transmissions. In conclusion, we believe none of the experiments conducted in this paper raise any ethical concerns.  

==> eval3.tex <==


\noindent \textbf{Compute Resource Consumption.} To understand the compute resource consumption of the 5G core VNFs, we register more users and observe how the vMem and vCPU consumption increases. For the control plane VNFs, only the number of users will play a role and not their SST. For the UPF, however, depending on the traffic pattern of the SST, the UPF will be processing different amounts of data. Therefore the SST will also be of importance.



==> intro.tex <==
The deployment of next-generation mobile networks is an ongoing effort that is gaining momentum. Compared with legacy Long Term Evolution (LTE), the Fifth Generation (5G) networks have been designed to accommodate a wide range of industry verticals with different Quality of Service (QoS) demands. Thus, the delivery of services in 5G takes place over logically isolated segments called ``network slices." %that have been tailored for specific use cases. %In order to systematically classify the requirements of different users, the Third Generation Partnership Project (3GPP) has standardized certain use cases by designating them Slice Service Types (SSTs)~\cite{3gpp23501}. These include, but are not limited to, enhanced Mobile Broadband (eMBB), Ultra Reliable Low Latency Communication (URLLC), massive Internet of Things (mIoT) and Vehicular to Everything (V2X) communications. 
%
%To achieve a Standalone (SA) 5G deployment is made up of a next generation Radio Access Network (RAN) and a decentralized core network. In LTE, the core functions were bound to proprietary hardware as Physical Network Functions (PNFs). %This resulted in a rigid deployment model that was difficult to scale and could not address more fine-grained QoS requirements. 
For the flexible deployment of network slices, 5G leverages Network Functions Virtualization (NFV) as a building block for its core network~\cite{ordonez2017network,yousaf2017nfv}. While Physical Network Functions (PNFs) were used in LTE, 5G mobile network functions are packaged as Virtual Network Functions (VNFs) deployed on top of Commercial off-the-Shelf (COTS) hardware. %This creates a decentralized deployment model that can scale upon demand from the Mobile Virtual Network Operators (MVNOs). 
%Complementary to NFV, SDN enables the near-real time provisioning of these 5G core VNFs to dynamically respond to the QoS requirements of specific use cases. 
%Network slices are constructed by service chaining these VNFs based on instance templates~\cite{3gpp28530} to customize the delivery to the use case.

%This step towards virtualization creates enterprise opportunities for service providers to enter the mobile network ecosystem. 
%Small-to-Medium Enterprises (SME) can build Software-as-a-Service (SaaS), Platform-as-a-Service (PaaS) and Network-Slice-as-a-Service~\cite{gsm2021official,atalay2022network,zhou2016network} business models to create custom 5G offerings for end users.
The adoption of NFV for facilitating 5G deployments creates an increasing demand for computing infrastructure that can scale efficiently. To fill this vacuum, cloud providers such as Amazon Web Services (AWS), Google Cloud Platform (GCP), and Microsoft Azure are starting to tailor Infrastructure-as-a-Service (IaaS) offerings for Mobile Virtual Network Operators (MVNOs). Proof-of-concept trials are being conducted by Swisscom and Ericsson to deploy the 5G core on top of AWS~\cite{Swisscom30online}. Furthermore, Deutsche Telekom~\cite{Deutsche96online} and Telefonica~\cite{Telefóni70online} have started partnerships with AWS and Azure to explore a cloud-based 5G core network.
%the latter cloud giant has further solidified partnerships with other Telecommunication Service Providers (TSPs). %Currently these include Verizon, KDDI, Vodafone, SK Telekom and Bell~\cite{AWSWavel60online}. 
Given these developments, the objective of this paper is to understand the latency overhead and throughput bottlenecks associated with carrying out large-scale 5G deployments using the AWS public cloud. We experiment with alternative edge location options in seven countries, across eight AWS regions. %The insight we provide can be leveraged by MVNOs 

The infrastructure of AWS is divided into geographical segments denoted as parent regions. As illustrated in Figure~\ref{fig:awsinfra}, each region consists of multiple Availability Zones (AZs) and, for chosen regions, finer-grained Local Zones (LZs)~\cite{Deployme40online}. 
While an AZ is a generic deployment zone that exists for reliability through redundancy, LZs exist to enable low-latency applications at the edge of the AWS network. In addition to AZs and LZs, AWS has introduced the ``Wavelength Zone"~\cite{AWSWavel60online} (WZ). The WZs deliver an integrated cloud environment capable of supporting Ultra Reliable Low Latency Communication (URLLC) 5G applications by providing AWS features at the 5G network edge. Compared to LZs, this is achieved by deploying specific applications directly on top of the Telecommunication Service Provider (TSP) infrastructure, in close proximity to the 5G Radio Access Network (RAN). However, due to this displacement, AZ-WZ connections are subject to a higher latency than their AZ-LZ counterparts. %We confirm this through our preliminary benchmarks during evaluation.

%All these zones offer compute resources in the form of Elastic Compute Cloud (EC2) instances~\cite{AmazonEC25online}. SMEs and MVNOs can leverage these flexible resources to deploy applications close to the network edge using LZs or specifically the 5G edge with WZs.

LZs and WZs are well-suited for hosting URLLC applications to enhance user plane Quality of Experience (QoE). In addition to user applications, they can be leveraged for deploying 5G core VNFs to minimize the control plane latency to the RAN.
%for cases that would benefit from it.
%Depending on the Slice Service Type (SST)~\cite{3gpp23501} of the use case,
%
%On the one hand, user plane latency and throughput are important for providing a good Quality of Experience (QoE). On the other hand, control plane latency can be crucial in maintaining reliability for Mission Critical Services (MCSs) such as healthcare, energy and robotics~\cite{borsatti2022mission}. %3GPP has started defining reliability requirements for such systems. 
%
The advent of moving 5G applications and core VNFs into a public cloud raises performance concerns at both the control and user planes.
Mission Critical applications with dense signaling require low latency in control plane handling~\cite{3gpp22280}. On the other hand, applications such as Augmented- and Virtual- Reality (AR/VR) require low latency in the user plane. 

The significance of prioritizing among these operational planes is illustrated in Figure~\ref{fig:aws5gdep}. Two network slices are depicted over a tentative 5G core deployment in a hybrid AZ, LZ, and WZ layout. For the Mission Critical slice 1, it is more important to manage the network slice setup and transfer times~\cite{3gpp22280} of the clients to maintain high reliability. Therefore, slice 1 is stretched out over an LZ-AZ connection, where the LZ-AZ latency is lower than the WZ-AZ alternative. This reduces the end-to-end operational time of interactions between the Serving Network (SN) (i.e., UPF, SMF, AMF) and the Home Network (i.e., AUSF, UDM, UDR). 
%
%This minimize the control plane latency between the Home Network VNFs (i.e., AUSF, UDM, UDR) and the Serving Network VNFs (UPF, SMF, AMF). 
On the other hand, for better QoS in latency-sensitive  applications such as enhanced Mobile Broadband (eMBB) and URLLC cases, the data session VNFs (i.e., SMF, UPF) are deployed closer to the 5G edge in WZs. Therefore, slice 2 is deployed over a WZ-AZ connection. 


%On the other hand, it is more important to manage the network slice setup and transfer times~\cite{3gpp22280} in order to maintain high reliability for Mission Critical Services (MCSs). Therefore, select VNFs (i.e., NRF AMF, SMF) need to be deployed closer to the on-premises applications while still maintaining minimal latency with the back-end management VNFs (i.e., AUSF, UDM, UDR). This way the latency of the high volume control plane traffic can be minimized. For this example, the control plane can be scaled by opting for an LZ edge instead of a WZ. %On the other hand, to deliver the best QoE for virtual reality (VR) applications in the enhanced Mobile Broadband (eMBB) and URLLC SST, the data session VNFs (i.e., SMF, UPF) need to deployed closer to the 5G edge in WZs.

%Our study quantifies the control plane latency overhead of critical 5G tasks and user plane bottlenecks in hybrid AZ, LZ and WZ deployments across multiple locations within AWS. Leveraging our findings, 
%The control and user plane trade-off between opting for an LZ or WZ edge is important to quantify so that 
%operators around the world can make informed decisions regarding their 5G deployments. The complexity increases further by considering the cost of computational resources and the data transfer at the edge locations. Currently, the flavor pool for AWS Elastic Compute Cloud (EC2)~\cite{AmazonEC25online} instances at edge zones are restricted to those with fewer CPUs. Hence, it will become necessary to provision more nodes to scale certain use cases. Hence, in addition to QoS, it is also crucial to understand the resource consumption of a full-fledged 5G core to optimize the deployment cost depending on instance availability.

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.24\columnwidth}
        \centering
        \includegraphics[width=\textwidth,trim={14.5cm 6.1cm 13.7cm 3cm},clip]{figures/awsinfra_sfont.pdf}
        \caption[]%
        {{\small }}    
        \label{fig:awsinfra}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.68\columnwidth}  
        \centering 
        \includegraphics[width=\textwidth,trim={7.9cm 4.6cm 9.5cm 2.2cm},clip]{figures/aws5gdepannot.pdf}
        \caption[]%
        {{\small }}    
        \label{fig:aws5gdep}
    \end{subfigure}
    \caption{(a) Breakdown of an AWS parent region with different infrastructure zones; (b) QoS-sensitive 5G deployment on top of AWS across AZs, LZs, and WZs}
    \label{fig:awsow}
\end{figure}

%\vspace{-2in}

To the best of our knowledge, this work is the first to shed light on large-scale 5G deployments over a public cloud at a global scale. Specifically, we quantify the control plane latency overhead of critical 5G tasks and user plane bottlenecks in hybrid AZ, LZ, and WZ deployments across multiple locations within AWS. Leveraging our findings, operators around the world can make informed decisions regarding their 5G deployments to determine favorable placements of control and user plane entities for different use cases. Our main contributions are summarized below.

%We report the latency overhead for control plane operations in a hybrid central/edge cloud environment. Additionally, our investigation demystifies performance bottlenecks that exist between LZs/WZs and AZs to determine favourable placements for 5G user plane entities (i.e., the UPF and 5G application servers) for different use cases.
%
%Furthermore, the innate flexibilibe ty of 5G deployments as a result of NFV, gives operators the ability to deploy specific core VNFs in foreign countries to facilitate roaming without changing infrastructure domains. For instance, an individual travelling from the United States to Argentina can use edge VNFs located in the Buenos Aires LZ, while using the Verizon central cloud VNFs deployed in Northern Virginia. Therefore it is critical to not only understand the implications of 5G cloud deployments for domestic cases with respect to an operator but also roaming scenarios that include international users. %Depending on the VNF deployment strategy being used, signalling across VNFs 
%
%Ultimately, our goal is to perform a deep dive into the QoS and compute consumption implications of deploying specific network slice VNFs at different cloud hierarchies within AWS. 

\begin{itemize}
    \item For finer-grained control over experimentation, we use the open-source OpenAirInterface~\cite{oaiopena76online} (OAI) 5G core and the gNBSIM~\cite{RohanGnb5online} RAN. This allows us to manage 5G deployments without relying on any proprietary solution. We create multiple self-managed Kubernetes clusters on top of Elastic Compute Cloud (EC2) instances spanning multiple zones. These clusters are used to instantiate mass end-to-end connections between emulated users and Data Network Nodes (DNNs) that we control. To perform analysis on a global scale, we conduct experiments in eight different parent regions for 18 different edge zones.
    \item We provide detailed measurements that demystify the performance aspects of the AWS edge compute network. This includes weekly benchmarks on latency, throughput and packets loss. Firmly establishing these benchmarks within AWS not only elevates our 5G core study, but will also prove valuable to other researchers that seek to utilize the same infrastructure. In the future, our benchmarks can serve as a timestamp for the evolving AWS architecture that other studies can leverage to make comparisons with.
    \item To evaluate the 5G control plane, we build a state-of-the-art instrumentation environment using Jaeger~\cite{Jaegerop88online} and OpenTelemetry~\cite{OpenTele38online}. Integrated into this ecosystem, our custom monitoring Side-car Proxy (SCP) sits adjacent to each VNF, collecting telemetry data. Through this pipeline, we are able to trace the HTTP transactions between individual Representational State Transfer (REST) APIs of the 5G core. %By deploying end-to-end sessions at different AWS AZs, LZs and WZs, the control plane latency overhead of 5G cloud deployments is analyzed. 
    In our evaluations, we derive and experiment with multiple control plane strategies pertaining to real-life use cases (e.g., MCS, URLLC). Each strategy is associated with a placement pattern, where VNFs are shuffled between an edge zone and an AZ. Comparing the overhead of different strategies, we provide insight into what the control plane latency implications are for cloud-based 5G deployments. %This includes experimenting with same and cross region AZs, LZs and WZs in order to investigate roaming scenarios across countries.

    \item To understand user plane bottlenecks in different regions, traffic loads of real-life 5G use cases are recorded. Then, we create end-to-end user connections across edge zones and AZs. The captured downlink and uplink traffic is replayed through the 5G user plane to create traffic on top of AWS. Through these experiments, we measure the bandwidth bottlenecks between edge zones and AZs. Our goal is to provide operators with guidance regarding 5G user plane entity placement (e.g., UPF and DNN) in the cloud.

\end{itemize}














==> measframe.tex <==
%The objective of the monitoring framework is to enable end-to-end HTTP transaction tracing within the 5G core control plane. To that end, an instrumentation pipeline is constructed using Jaeger and OpenTelemetry. This section presents the design overview of the framework followed by the message flow between the entities.

%\subsection{System Overview}
We build a monitoring framework to conduct HTTP transaction tracing within the 5G core control plane. In particular, an instrumentation pipeline is constructed using Jaeger and OpenTelemetry as illustrated in Figure~\ref{fig:frameov}. To highlight the overall flow of the system, each building block is shown within its respective deployment hierarchy in the experimentation environment. For a Kubernetes cluster, this deployment can occur at a pod-, node- or cluster-level. %depending on the role of the component. %We can classify this deployment into three logical domains. These are the 5G core network components, OpenTelemetry SCPs along with agents and finally the Jaeger deployment. 

Deployed in individual pods, 5G core VNFs are the applications of interest that are traced by the monitoring framework. Each VNF is comprised of multiple microservices dedicated to a specific core network operation. To avoid having to modify the source code of the VNFs for gathering telemetry information, we design a custom SCP for intercepting and redirecting the HTTP messages between the 5G pods. This is denoted as indirect communication and has been standardized by 3GPP in Release 16 as a viable VNF-to-VNF interaction method. More details about the message interception are provided in Appendix~\ref{app:msginterflow}.

\begin{comment}
    
\begin{figure}[t]
\begin{minipage}[b]{0.45\columnwidth}
    \includegraphics[width=0.95\columnwidth,trim={11.1cm 5.4cm 10.5cm 3.4cm},clip]{figures/monovs.pdf}
     \caption{Overview of the monitoring framework for 5G core transaction tracing}
     \label{fig:frameov}
\end{minipage}\hfill % maximize horizontal separation
\begin{minipage}[b]{0.54\columnwidth}
    \includegraphics[width=\columnwidth,trim={8.8cm 10.3cm 11.5cm 6.5cm},clip]{figures/framemsg.pdf}
     \caption{Sample API call from AMF to SMF illustrating monitoring SCP interception}
     \label{fig:framemsg}
\end{minipage}
\end{figure}
\end{comment}

\begin{comment}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth,trim={3.3cm 9.7cm 3.8cm 3.2cm},clip]{figures/monovshor.pdf}
     \caption{Overview of the monitoring framework for 5G core transaction tracing}
     \label{fig:frameov}
\end{figure}
\end{comment}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth,trim={11.1cm 4.3cm 10.5cm 2.8cm},clip]{figures/monovs.pdf}
     \caption{Overview of the monitoring framework for 5G core transaction tracing}
     \label{fig:frameov}
\end{figure}


Sitting adjacent to each 5G core VNF in the pod is the monitoring SCP designed using OpenTelemetry. %We generate the necessary logs for our control plane measurements by ine. 
The SCP functions as a two-way redirection proxy that forwards messages to and from the 5G application residing in the same pod. When a message enters the pod network sandbox, it is processed at the OpenTelemetry HTTP server within the SCP. As the HTTP request is forwarded to its destination, a span is created for the given transaction based on the 5G CAPIF path in the URL. This allows us to distinguish between individual 5G core control plane messages and identify sender/receiver VNFs. Once the spans are created, the SCP sends them to the node-level OpenTelemetry agent. 

The OpenTelemetry agent functions as the initial consolidation point for the gathered logs. After receiving telemetry from individual SCPs, it forwards the information to the respective Jaeger agent deployed alongside it. A central Jaeger collector receives logs from all the Jaeger agents in the cluster and stores them in a Cassandra database as JSON files. Finally, the Jaeger query is used to fetch them from the database. Both OpenTelemetry and Jaeger agents are deployed as Daemonsets within the Kubernetes cluster, and communications with them take place over Kubernetes DNS.


\begin{comment}
\subsection{Message Interception Flow}

To clarify the message interception process in our monitoring pipeline, Figure~\ref{fig:framemsg} depicts a sample message flow for a single HTTP transaction taking place between AMF and SMF. The gray outline corresponds to individual pod deployments within the Kubernetes cluster. The IPTABLES of all the pods have been modified to perform port forwarding on all messages originating from the user identifier (UID) of the 5G core VNFs. Therefore, every outgoing and incoming message to the VNFs is redirected through the monitoring SCP.

In this example, AMF is making an API call to SMF with the CAPIF path $/nsmf- pdusession$ on port 80. The pod network sandbox redirects this HTTP request to the localhost on port 10096, where the monitoring SCP is running an OpenTelemetry HTTP server. Upon receiving the request, SCP extracts the CAPIF path from the URL and creates a span corresponding to the specific source and destination VNF (i.e., AMF and SMF, respectively). Finally, it changes the destination port on the outgoing message and forwards it to the pod of the target VNF. The same process is executed within the SMF pod upon the arrival of the HTTP message. Combining this interception and redirection with the instrumentation pipeline in Figure~\ref{fig:frameov} allows us to perform distributed tracing on the HTTP transactions in the 5G core. Ultimately, we are able to monitor the end-to-end execution time of individual operations and group them together in concise logs. 
\end{comment}

 

